LIO*: Low Level Information Flow Control in F*

We present Labeled Input Output in F* (LIO*), a verified framework that enforces information flow control (IFC) policies developed in F* and automatically extracted to C. Inspired by LIO, we encapsulated IFC policies into effects, but using F* we derived efficient, low level, and provably correct code. Concretely, runtime checks are lifted to static proof obligations, the developed code is automatically extracted to C and proved non-interferent using metaprogramming. We benchmarked our framework on three clients and observed up to 54% speedup when IFC runtime checks are proved statically. Our framework is designed to aid development of embedded devices where both enforcement of security policies and low level efficient code is critical.

==> Makefile <==
###
### generic GNU make Makefile for .tex -> .pdf.
### ransford at cs.washington.edu
###   http://github.com/ransford/pdflatex-makefile
###
### Recommended usage:
###   1. echo 'include Makefile.include' > Makefile
###   2. Optional: Edit the Makefile to override $(TARGET)
###      and anything else (e.g., PDFVIEWER, AFTERALL)
###   3. $ make snapshot
###      # pass around a draft...
###   4. $ make distill
###      # submit the camera-ready version with embedded fonts
###
### Final result:
###   % cat Makefile
###   TARGET=mypaper
###   PDFVIEWER=open -a 'Adobe Acrobat Professional'
###   AFTERALL=mypostprocessingstep
###   include Makefile.include
###
###   mypostprocessingstep:
###           # do something...
###

PDFLATEX	?= pdflatex -halt-on-error -file-line-error -shell-escape
BIBTEX		?= bibtex
MAKEGLOSSARIES ?= makeglossaries
MAKENOMENCL ?= makeindex

## String to find in log to check whether rerun is necessary
RERUN_PATTERN = Rerun to

ifneq ($(QUIET),)
PDFLATEX	+= -interaction=batchmode
ERRFILTER	:= > /dev/null || (egrep ':[[:digit:]]+:' *.log && false)
BIBTEX		+= -terse
else
PDFLATEX	+= -interaction=nonstopmode
ERRFILTER=
endif

## Action for 'make view'
OS=$(shell uname -s)
ifeq ($(OS),Darwin)
PDFVIEWER	?= open
else
PDFVIEWER	?= xdg-open
endif

## Name of the target file, minus .pdf: e.g., TARGET=mypaper causes this
## Makefile to turn mypaper.tex into mypaper.pdf.
TARGETS += $(TARGET)
TEXTARGETS = $(TARGETS:=.tex)
PDFTARGETS = $(TARGETS:=.pdf)
AUXFILES   = $(TARGETS:=.aux)
LOGFILES   = $(TARGETS:=.log)

## Inkscape SVG file processing:
ifeq ($(shell which inkscape >/dev/null 2>&1 && echo USING_INKSCAPE),USING_INKSCAPE)
  FIG_SVG=$(wildcard $(FIGS)/*.svg)
  FIG_PDF=$(FIG_SVG:.svg=.pdf)
else
  FIG_PDF=
endif

## If $(TARGET).tex refers to .bib files like \bibliography{foo,bar}, then
## $(BIBFILES) will contain foo.bib and bar.bib, and both files will be added as
## dependencies to $(PDFTARGETS).
## Effect: updating a .bib file will trigger re-typesetting.
BIBFILES += $(patsubst %,%.bib,\
		$(shell grep '^[^%]*\\bibliography{' $(TEXTARGETS) | \
			grep -o '\\bibliography{[^}]\+}' | \
			sed -e 's/^[^%]*\\bibliography{\([^}]*\)}.*/\1/' \
			    -e 's/, */ /g'))

## Add \input'ed or \include'd files to $(PDFTARGETS) dependencies; ignore
## .tex extensions.
INCLUDEDTEX = $(patsubst %,%.tex,\
		$(shell grep '^[^%]*\\\(input\|include\){' $(TEXTARGETS) | \
			grep -o '\\\(input\|include\){[^}]\+}' | \
			sed -e 's/^.*{\([^}]*\)}.*/\1/' \
			    -e 's/\.tex$$//'))

AUXFILES += $(INCLUDEDTEX:.tex=.aux)

## grab a version number from the repository (if any) that stores this.
## * REVISION is the current revision number (short form, for inclusion in text)
## * VCSTURD is a file that gets touched after a repo update
SPACE = $(empty) $(empty)
ifeq ($(shell git status >/dev/null 2>&1 && echo USING_GIT),USING_GIT)
  ifeq ($(shell git svn info >/dev/null 2>&1 && echo USING_GIT_SVN),USING_GIT_SVN)
    # git-svn
    ifeq ($(REVISION),)
      REVISION := $(shell git svn find-rev git-svn)
    endif
    VCSTURD := $(subst $(SPACE),\ ,$(shell git rev-parse --git-dir)/refs/remotes/git-svn)
  else
    # plain git
    ifeq ($(REVISION),)
      REVISION := $(shell git describe --always HEAD)
    endif
    GIT_BRANCH := $(shell git symbolic-ref HEAD 2>/dev/null)
    VCSTURD := $(subst $(SPACE),\ ,$(shell git rev-parse --git-dir)/$(GIT_BRANCH))
  endif
else ifeq ($(shell hg root >/dev/null 2>&1 && echo USING_HG),USING_HG)
  # mercurial
  ifeq ($(REVISION),)
    REVISION := $(shell hg id -i)
  endif
  VCSTURD := $(subst $(SPACE),\ ,$(shell hg root)/.hg/dirstate)
else ifeq ($(shell svn info >/dev/null && echo USING_SVN),USING_SVN)
  # subversion
  ifeq ($(REVISION),)
    REVISION := $(subst :,-,$(shell svnversion -n))
  endif
  VCSTURD := $(addsuffix /.svn/entries, $(shell svn info | grep 'Root Path' | sed -e 's/\(.*\:\)\(.*\) /\2/'))
endif

# .PHONY names all targets that aren't filenames
.PHONY: all clean pdf view snapshot distill distclean

all: pdf $(AFTERALL)

ifeq ($(shell which inkscape >/dev/null 2>&1 && echo USING_INKSCAPE),USING_INKSCAPE)
$(FIGS)/%.pdf: $(FIGS)/%.svg  ## Figures for the manuscript
	inkscape -C -z --file=$< --export-pdf=$@ 2> /dev/null
endif

pdf: $(FIG_PDF) $(PDFTARGETS)


view: $(PDFTARGETS)
	$(PDFVIEWER) $(PDFTARGETS)

# define a \Revision{} command you can include in your document's preamble.
# especially useful with e.g. draftfooter.sty or fancyhdr.
# usage: \input{revision}
#        ... \Revision{}
ifneq ($(REVISION),)
REVDEPS += revision.tex
revision.tex: $(VCSTURD)
	echo '\newcommand{\Revision}'"{$(subst _,\_,$(REVISION))}" > $@
AUXFILES += revision.aux
endif

# to generate aux but not pdf from pdflatex, use -draftmode
%.aux: %.tex $(REVDEPS)
	$(PDFLATEX) -draftmode $* $(ERRFILTER)

# specify KEEPAUX=1 if you need to keep auxiliary (.aux) files for some other
# tool (e.g., an autocompleting text editor)
ifneq ($(KEEPAUX),1)
  .INTERMEDIATE: $(AUXFILES)
endif

# introduce BibTeX dependency if we found a \bibliography
ifneq ($(strip $(BIBFILES)),)
BIBDEPS = %.bbl
%.bbl: %.aux $(BIBFILES)
	$(BIBTEX) $*
endif

# introduce makeglossaries dependency if we found \printglossary/ies
HAS_GLOSSARIES = $(shell \
		grep '^[^%]*\\printglossar\(ies\|y\)' $(TEXTARGETS) $(INCLUDEDTEX) && \
		echo HAS_GLOSSARIES)
ifneq ($(HAS_GLOSSARIES),)
GLSDEPS = %.gls
%.gls: %.aux
	$(MAKEGLOSSARIES) $(TARGETS)
endif

# introduce makenomenclature dependency if we found \printnomenclature
HAS_NOMENCL = $(shell \
		grep '^[^%]*\\printnomenclature' $(TEXTARGETS) $(INCLUDEDTEX) && \
		echo HAS_NOMENCL)
ifneq ($(HAS_NOMENCL),)
NLSDEPS = %.nls
%.nls: %.nlo
	$(MAKENOMENCL) $(TARGETS).nlo -s nomencl.ist -o $(TARGETS).nls
endif

$(PDFTARGETS): %.pdf: %.tex %.aux $(GLSDEPS) $(BIBDEPS) $(INCLUDEDTEX) $(REVDEPS) $(NLSDEPS)
	$(PDFLATEX) $* $(ERRFILTER)
ifneq ($(strip $(BIBFILES)),)
	@if egrep -q "undefined (references|citations)" $*.log; then \
		$(BIBTEX) $* && $(PDFLATEX) $* $(ERRFILTER); fi
endif
	@while grep -q "$(RERUN_PATTERN)" $*.log; do \
		$(PDFLATEX) $* $(ERRFILTER); done

DRAFTS := $(PDFTARGETS:.pdf=-$(REVISION).pdf)
$(DRAFTS): %-$(REVISION).pdf: %.pdf
	cp $< $@
snapshot: $(DRAFTS)

%.distilled.pdf: %.pdf
	gs -q -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ \
		-dCompatibilityLevel=1.5 -dPDFSETTINGS=/prepress -c .setpdfwrite -f $<
	exiftool -overwrite_original -Title="" -Creator="" -CreatorTool="" $@

distill: $(PDFTARGETS:.pdf=.distilled.pdf)

distclean: clean
	$(RM) $(PDFTARGETS) $(PDFTARGETS:.pdf=.distilled.pdf) $(EXTRADISTCLEAN)

clean:
	$(RM) $(foreach T,$(TARGETS), \
		$(T).bbl $(T).bcf $(T).bit $(T).blg \
		$(T)-blx.bib $(T).brf $(T).fdb_latexmk \
		$(T).fls $(T).glg $(T).glo $(T).gls \
		$(T).glsdefs $(T).glx \ $(T).gxg \
		$(T).gxs $(T).idx $(T).ilg $(T).ind \
		$(T).ist $(T).loa $(T).lof $(T).lol \
		$(T).lot $(T).maf $(T).mtc $(T).nav \
		$(T).out $(T).pag $(T).run.xml $(T).snm \
		$(T).svn $(T).tdo $(T).tns $(T).toc \
		$(T).vtc $(T).url) \
		$(REVDEPS) $(AUXFILES) $(LOGFILES) \
		$(EXTRACLEAN) $(FIG_PDF)
cleansmall:
	$(RM) $(foreach T,$(TARGETS), \
		$(T).bcf $(T).bit $(T).blg \
		$(T)-blx.bib $(T).brf $(T).fdb_latexmk \
		$(T).fls $(T).glg $(T).glo $(T).gls \
		$(T).glsdefs $(T).glx \ $(T).gxg \
		$(T).gxs $(T).idx $(T).ilg $(T).ind \
		$(T).ist $(T).loa $(T).lof $(T).lol \
		$(T).lot $(T).maf $(T).mtc $(T).nav \
		$(T).out $(T).pag $(T).run.xml $(T).snm \
		$(T).svn $(T).tdo $(T).tns $(T).toc \
		$(T).vtc $(T).url) \
		$(REVDEPS) $(AUXFILES) $(LOGFILES) \
		$(EXTRACLEAN) $(FIG_PDF)


==> proof.tex <==
%\section{Generating theorem statements}
\section{Theorems generation and proofs}
\label{section:metathery}

This section experiences the mechanized simulation proof of \gls{liostar} using \gls{metastar}, that is realised on a per-program basis.
%
The problem addressed here is that our \gls{liostar} system is ``working correclty'': no unexpected leakage of information should ever happen; the IFC policy the used spelled out should be respected at every state of the program.
More formally, a good \gls{ifc} system should enjoy \textit{non-interference}.

\subsection{Motivation}

\cite{stefan:2017:flexible} and \cite{Parker:2019:LIF:3302515.3290388} describe proofs of \gls{lio} systems using the Coq theorem prover and Liquid-Haskell.
These proofs are expressed by considering the lambda-calculus equipped with \gls{lio} primitives, instead of the programming language at stake.
They are performed by proving a behavioral simulation relation between \gls{lio} programs and erased programs.
These proofs hence apply to \gls{lio}, not to its particular implementation (i.e., the executable Haskell code).

On the contrary here, the aim is to prove that the actual implementation, and not a model of it, enjoys non-interference.
For this we define a meta-program that, given a \gls{fstar} program, spells out a non-interference theorem
w.r.t.\ \gls{liostar}.
%\jp{(translation validation CITE PNUELI) ?}.

The benefit of our approach is that a per-program theorem both requires lighter human effort than a generic one, and can further help in validating security of the target application with certification authorities.
Moreover, instead of proving this property on an idealized lambda calculus, our solution generates theorem statements that directly apply on \gls{fstar} programs. 

\subsection{Non-interference}
An \gls{ifc} system should respect non-interference. In order to express that property, two prior notations are required:
\begin{itemize}
\item for $x$ a value and $l$ a label, $x^l$ projects $l$-tagged data present in $x$;
\item for $x, y$ values, $l$ a label, $x =_l y = \forall l' \sqsubseteq l, x_{l'} = y_{l'}$. 
\end{itemize}

\noindent Non-interference can then be spelled out as \(\forall x\,y\,l,   x =_l y \implies f~x =_l f~y  
\).

However, the projection of a value
%\jp{which one ?}\lf{\small actually, it is just the projection of a value, it just results in a part of the given value, so I guess removing ``part of'' would disambiguate the sentence, what do you think?}
with respect to a given label is, in general, not well-defined.
Hence, we adopt a more pragmatic (and computable) approach, with a conventional notion of erasure.
The erasure of a \textit{term} $t$ relative to the label $l$ realizes the idea behind $t^l$:
it is a transformation of the term where every labeled information is replaced by a placeholder, that acts as a black box.
For instance, consider the term $\lambda x\,y\mapsto x + y$.
Supposing $x$ is always a labeled integer with the label |High|, and $y$ always labeled as |Low|, we have:
\[
\mathit{erase}_{Low}\left(\lambda x\,y\mapsto x + y\right) = \left( \lambda x\,y\mapsto \bullet + y\right) = \lambda x\,y\mapsto\bullet
\]

Note that the placeholder, denoted $\bullet$, is absorbant: certain total operations involving this placeholder should result in $\bullet$, a black hole, as well.
However, this absorbance property should be carefully designed.
Consider the function $f = \lambda x\ y \mapsto y$ and the addition function $(+)$.
$f\ \bullet$ shall not reduces to $\bullet$ ---$f$'s first argument does not contaminates its outcome, whereas $\bullet + 4$ shall reduce to $\bullet$ ---one is not able to observe a property on the outcome that depends only on $4$.

This notation of contaminant is important: the addition on $\mathbb{Z}$ is contaminant in both of its arguments.
However, consider the contaminance of multiplication on its first argument.
There exists a $y$, namly $y=0$, such that the ``is null'' observation is independent of $x$, on the expression $x * y$.
Indeed, semantically, this expression equals to $0$.
Contaminance is therefore a non-trivial property, that should be treated with extra care.

Formally, a function $f:\alpha\to\beta\to\gamma$ is contaminant whenever the following holds.
\lf{todo, double check this}

\vspace{-.5em}
\begin{equation}
 % \begin{split}
    \forall~
    (P: \alpha\to\beta\to\gamma)~
    (a: \alpha)~
    (b: \beta)
    ,~~~~~
    P~(f\ a\ b) \implies \left(
   \begin{array}{cl}
     &
        \exists a',~
        \neg P~(f\ a'\ b)
      \\
      \vee
      &
        \forall a'\ b',~
        P~(f\ a'\ b')
   \end{array}
    \right)
 % \end{split}
\end{equation}

Note that constructor of inductive types are not contaminant in any parameter in general.
However, if an inductive admit exactly one $n$-ary constructor, it should be considered as contaminant if $n-1$ of its arguments are computationally irrelevant.
This happen to be the case for the one constructor for the record $\mathit{labeled}$ of \gls{liostar}: 
it is contaminant, since its label is computationally irrelevant.
\lf{Note: if C unique constructor of T, then `C * *` should reduce to `*` as well. Should we say that?}

In our \gls{fstar} implementation, $\bullet$ is an axiomatized polymorphic value, and absorbance is axomatized for every contaminant function.
Below is the definition of $\bullet$ ---|placeholder| in the code snippet, along with the axomatization that the addition absorbs $\bullet$.
Note that defining some |placeholderAbsorbantPlus_left| is not necessary:
\gls{fstar} knows that addition is commutative. 

\begin{mcode}\label{placeholde_f_def}
assume val placeholder: (#a: Type) -> a
let placeholderAbsorbantPlus_left n : Lemma (placeholder + n == placeholder) = admit ()
\end{mcode}

\def\eval{\downarrow\!\!}
Non-interference can be expressed in terms of erasure and proved by simulation.
This amounts to comparing the evaluation of two versions of the same program that are erased at different times, where $\eval\cdot$ is the evaluation:

\vspace{-.5em}
\begin{equation}\label{eqn:sim}
  \mathit{erase}_l \eval f = \mathit{erase}_l \eval \left(\mathit{erase}_l~f\right)
\end{equation}

\subsubsection{\gls{metastar} formulation}

The Equation~\ref{label{eqn:sim}} however does not apply exactly in our approach:
in our scenario, there exists a fundamental difference between \textit{erasing a value} and \textit{erasing a term}.

\paragraph{Erasing a value}\label{subsub:par:erase-val} Let a type $\tau$ 
\begin{enumerate*}
\item that is not an arrow type (i.e. $\tau=\alpha\to\beta$ is forbidden) and
\item whose kind is not an arrow type either (i.e. $\tau=\mathit{either}$ is forbidden since $\tau:\mathit{Type}\to\mathit{Type}\to\mathit{Type}$)
\end{enumerate*}.
For instance, $\tau=\lambda\alpha. \mathit{option}~\alpha$ is forbidden, while $\tau=\mathit{option}~\mathbb{Z}$ is allowed:
otherwise, an unattended labeled type could sneak in $\tau$.

Then the function $\epsilon_\tau$ is a value-eraser, that is a total function of type $\mathit{label}\to\tau\to\tau$. $\epsilon_\tau$ behaves as the identity if $v:\tau$ cannot hold any labeled information due to its type defintion $\tau$.
However, if $\tau$ structurally contains  $\mathit{labeled}~\alpha$ (for some $\alpha$), $\epsilon_\tau$ will map every labeled value to their erased counterparts.
The code snipped below shows an example of value-eraser for the type $list~(option~(labeled~\mathbb{Z}))$.
Note that $eraseLabel$ is defined later in \S~\ref{def:erasedLabel}.

%\begin{figure}[ht]
\begin{mcode}[mathescape=$$]
let rec $\epsilon_{list~(option~(labeled~\mathbb{Z}))}$ (l: label) = match x with
  | Cons hd tl -> Cons (match hd with | Some x -> Some (eraseLabel l x) | None -> None)
                  ($\epsilon_{list~(option~(labeled~\mathbb{Z}))}$ tl)
  | Nil -> Nil
\end{mcode}
%\label{code:value-eraser-ex}
%\end{figure}

\paragraph{Erasing a term} A term-eraser function is of type $\term\to\term$.
A $\term$ is the meta-representation of an \gls{fstar} value.
Getting a $\term$ out of a \gls{fstar} value is an effectful operation, just as declaring a toplevel function:
one can understand quotation or toplevel declarations as monadic operations on the typechecker's state.
For Haskellers, the parralel can be done with Template Haskell, where meta programs lives in the monad $Q$. % TODO: if we speak about Tac, put here

Therefore, transforming a value to a term with quotation happens only once, at the same time declarations are processed.
The same observation holds for crafting ---via term transformations--- an erased version of some toplevel function.

Due to this timing setting, it is not wishable for the erased version a toplevel to be erased with a specific label in mind.
The label at which values should turn to $\bullet$ should be dynamic, and quantified universally when spelling out the theorem.
Due to that fact, the erased version $f'$ of a toplevel $f:\tau$ is of type $f':\mathit{label}\to\tau$.
The erased versions of toplevels see their type and definition prepend with a label.  

\paragraph{Rephrasing the theorem}

Spelling out the non-interference of a function $f: \alpha \to \beta$ %in our framework
yields the equation \ref{eqn:sim-meta}, where $f_\epsilon:\mathit{label}\to\alpha\to\beta$ is the meta-generated erased version of $f$.

\vspace{-.5em}
\begin{equation}\label{eqn:sim-meta}
  \forall (l:label)~(x:\alpha),~~~
  \epsilon_\beta~l~\left(f\ x\right)
  =
  \epsilon_\beta~l~
  \left(
    f_\epsilon~l~x
  \right)
\end{equation}

\subsection{Generation of value-erasers}\label{sub:generation-value-erasers}
This section treat of the generation of value eraser.
We achive this job in a generic programming manner: for every inductive or primitive type, we generate a parametric value-eraser.

\paragraph{The specific case}\label{def:erasedLabel}
As a basis, we define the $erasedLabel$ function as in the code snippet below:

\begin{mcode}
let eraseLabeled (vl:labeled $\alpha$) l =
  if vl.tag $\sqsubseteq $l then vl else { data=placeholder; tag=vl.tag }
\end{mcode}

\paragraph{Inductive type}
Let $\tau$ an inductive type with $n$ type arguments $\alpha_1\dots\alpha_n$.
We generate a function $\mathit{eraser}_\tau$ of type
$(\alpha_1\to\alpha_1)\to\dots\to(\alpha_n\to\alpha_n)\to\tau~\alpha_1\dots\alpha_n\to\tau~\alpha_1\dots\alpha_n$.

Recall the type restriction defined in~\ref{subsub:par:erase-val}:
value-eraser should work only on fully applied non-arrow types.
This is the reason why $\mathit{eraser}_\tau$ takes $n$ other erasers.

However, $\mathit{eraser}_\tau$ need to be called with proper erasing functions:
for instance, the identity function is not a correct eraser for the type $\mathit{labeled}\ \mathbb Z$.
Therefore, the direct use of $\mathit{eraser}_\tau$ is not left to the end user:
instead, type classes are used to resolve the proper functions when needed.
The resolved functions have been generated automatically, and thus implements the correct behaviour.
The end user interface to the eraser is |erase_value : 'l -> 'a -> 'a|.

\paragraph{Primitive types}
For primitive types (like $\mathbb B$, $\mathbb Z$ or $\mathit{unit}$), we define erasure by the identity function. 

\paragraph{Wrapping up}
For every elligible type $\tau$, the end-user can run a meta program to generate definitions so that $\epsilon_\tau:\mathit{label}\to\tau\to\tau$ is a value-eraser for $\tau$.    

\subsection{Erasing labeled values in terms}
Section~\ref{sub:generation-value-erasers} defined a way for generating a value-eraser per type, this subsection defines a meta program that transforms a term in an other.
The outcome term is such that every of its subterms are wrapped in a $\mathit{erasedLabel}$ call whenever it is possible.

\subsubsection{Is subterm wrappable?}
When analysing a subterm $t$ of a program, we need to know if $t$ shall be replaced with $mathit{erasedLabel}~t$: we need some kind of type discrimination.

To perform this type discrimination, we apply a straightforward recipe:
if $\mathit{eraseLabeled}~t~l$ (for some label $l$) type-check, it means $t$ was a labeled value.

To get rid of bounded variable issues (the subterm $x$ from $\lambda x\mapsto x$ won't typecheck: $x$ is not bound), we use a specific methodology.
While browsing a term, we always keep a backtracking function.
For every subterm $t'$ of a toplevel term $t$, we hand a function ---say $\Delta$--- that reincorporate $t'$ as a subterm of $t$, at the right place.
Then, instead of typechecking $\mathit{eraseLabeled}~t'~l$, we typecheck $\mathit{eraseLabeled}~(\Delta~t')~l$.

\subsubsection{Erasing a toplevel definition}

From a toplevel definition, we generate an alternative, erased, top-level definition.
If this function is |main|, it is unlikely to be self-contained. 
%
%Suppose one wants to get an erased version of its program that lives in the toplevel definition $main$: it's unlikely $main$ is self-contenant; one probably divided its program in multiple toplevel definitions and possible over multiple modules.
%
Therefore, if we generate the erased |main|, we should also generate erased-version of every functions it calls, and replicate this change in |main|.
However, as explained in \ref{tc-undecidable}, when erasing a term $t$, we need to have access to a type-checkable parent term.
Therefore, we cannot replace top-level names with erased name \textit{during the transformation}:
this replacement should take place at the end of the transformation.

Given a top-level definition $D$, we derive a list $D_{dep}$ of top-level dependencies, and so on for every top-level function in $D_{dep}$.
Then, we browse the AST of every top-level term |let d = t| discovered in $D_{dep}$, and apply the $\mathit{eraseLabeled}$ function to each subterm, using the type-checking strategy.
Erasing a term is done up to a given label: instead of generating the toplevel |let d_erased = t|, we generate |let d_erased eraseAtLabel = t eraseAtLabel|.
To finalize the generation of a toplevel term, we still need to replace every free variable so that they point to their erased version:
we browse each AST again, and instead of replacing a free variable $f$ with $f_{erased}$, we replace it with $f_{erased}~\mathit{eraseAtLabel}$.

\subsubsection{Generating axioms for placeholders}
As explained in~\ref{placeholde_f_def}, $n$ axioms should be generated for every $m$-ary ($n\leq m$) functions that are contaminant in their $n$ arguments.
This can be tedious and error prone to write these by hand.

Thus, we propose a meta program |make\_absorbant\_axioms|, that, given a list of toplevel names, forges multiple axiomatized lemmas about absorbance for $\bullet$, for every parameters of every functions.

Lemmas in \gls{fstar} can have a SMT pattern clause:
this clause tells the SMT solver to apply certains lemmas when it sees certains term patterns.
However, the current \gls{metastar} API does not support manipulating these; we therefore made a very simple patch so that it supports it.

\subsubsection{Theorem generator}
The theorem generator is a meta-program that takes a top-level definition and produces a proposition.
It addresses the sensitive point of the meaning and evaluation of equation \ref{eqn:sim} in \gls{metastar}.
For a given term, evaluation is exactly normalization: erasing a term after normalization is to be seen as erasing the result of the computation performed by the term.
For instance, erasing |label 2 L * 21| after normalization is exactly the same as normalizing |label 42 L|.
Instead, erasing this same term without prior normalization results in |label 2 H * 21|.
This subtlety is the core idea of our proof by simulation.

\paragraph*{Effect} A \gls{liostar} computation lives in a specific effect.
Normalization over an effect-full computation has not the desired behaviour:
indeed, in general, an effect might mean side-effects (e.g. memory state transformation), and normalization should be a pure process.
Therefore, before normalizing a \gls{liostar} computation, one should \textit{reify} it, that is, interpreting the computation as a pure function.
%For instance, if the effect has a primitive providing randomness source, one can model it as a pure function that operates on a given infinite list of number. ???

\paragraph*{Outlook} Our implementation of simulation theorems meets the objectives of carefully translating the equation \ref{eqn:sim}, keeping in mind the subtleties about effect-full operations and meta normalization in \gls{metastar}.

\subsection{Illustration}
Reconsider the |checkLabeled| and |eqLabeled| functions, first introduced in \S~\ref{ss:deiansloi}. To erase |checkLabeled| and |eqLabeled|, one should write the following \textit{splice} ---that is a meta-program that generates one or multiple toplevel definitions:

% The '%' in the following code snippet is intended:
% this is F* syntax for running splices!
\begin{mcode}
%splice[add_erased, checkLabeled_erased] (mk_erased_toplevel (lookup (`checkLabeled)))
\end{mcode}

In our example, |mk_erased_toplevel| crafts the following definitions:

\begin{mcode}
let eqLabeled_erased (lErase: 'l) (v1 v2:labeled 'a)
	: Ifc bool
= let i1 = unlabel (eraseLabeled lErase v1) in
  let i2 = unlabel (eraseLabeled lErase v2) in
  i1 = i2
        
let checkLabeled_erased (lErase: 'l) (l:'l) (i:'a) (lv:labeled 'a): Ifc bool
	(requires fun l0 -> reveal l0 `canFlow` l)
	(ensures ...)
	= let lv1 = eraseLabeled lErase (label v l) in
          eqLabeled_erased lErase (eraseLabeled lErase lv) (eraseLabeled lErase lv1)
\end{mcode}

\lf{very quick and fast writing here, so sorry for mispellings or not very clear sentences, I ll have to double check it tomorrow}

Here, a few things are worth noticing:
\begin{enumerate*}
\item generating |checkLabeled_erased| generates as well |eqLabeled_erased|
\item every of these erased functions takes one supplementary parameter |lErase|, in comparaison to their original counterparts
\item this argument is passed around consistantly
\item every subterm in the functions bodies that have a labeled type is wrapped with |eraseLabeled|
\end{enumerate*}.

Note that these functions are still living in the IFC effect.
Our goal is to formulate two non-interference theorems:
for every possible input values and state, these functions should be non-inteferent.

The first step is to bring these IFC computations as total computations, by the mean of reification.
Doing so transforms an IFC computation in a (pure) context transformer.
For instance, reifying the IFC function |fun n -> n + 3| would produce the function |fun n ctx -> n + 3, ctx|. 

Notice that the reification of a IFC computation that produces |'a|s is a pure computation that produces tuples of |'a|s and |context|s.
Recall what our IFC context is made of:
basically, a current label.
We shall therefore consider this current label in our erasure scheme.
A |'a $\times$ context| value should be transformed into a labeled value |labeled 'a|: |getResult|, below, achieve this.

For $n$ a non null natural number, |reify$n$| reifies then erase (with |erase_value| and |getResult|)- $n$-ary computations, while |reify$n$'| does the same thing, but with erased versons of |N| ary-computations.

Finaly, |reifyN| is a meta-program that finds the correct |reify$n$| or |reify$n$'| for a its given parameter.

As an example, here is the definition for these functions with $n=2$, along with |getResult| implementation.

\begin{mcode}
let getResult (x: 'a * context): labeled 'a
  = mkLabel (fst x) (snd x).cur

let reify2'
  #a #b #ret #wp
  [| hasEraser ret |]
  ($\$$f: (lErase: labelType) -> (x: a) -> (y: b) -> IFC ret (wp x y))
  (lErase: 'l) (c0: context) (x: a) (y: b {wp x y c0 (fun _ -> True)})
  : Tot (labeled ret)
  = fun lErase c0 x y -> erase_value lErase (getResult (reify (f lErase x y) c0))
  
let reify2
  #a #b #ret #wp // For every input and output types, and any weakest precondition
  [| hasEraser ret |] // $\color{gray_ulisses}eraser_{\mathit{ret}}$ should exist
  ($\$$f: (x: a) -> (y: b) -> IFC ret (wp x y)) // we take a IFC computation
  (lErase: 'l) (c0: context) (x: a) (y: b {wp x y c0 (fun _ -> True)})
  : Tot (labeled ret)
  = erase_value lErase (getResult (reify (f x y) c0))
\end{mcode}

We are now all set to spell out non-interference:
\begin{mcode}
let eqLabeled_NI l x y c0
   : Lemma (reifyN eqLabeled_erased l x y == reifyN eqLabeled l x y)
   = ()
 
let checkLabeled_NI lE l i lv (c0: context {reveal c0 `canFlow` l})
   : Lemma (reifyN checkLabeled_erased lE l i lv == reifyN checkLabeled lE l i lv)
   = ()
\end{mcode}

\lf{NOTE: erasing arguments is messing up in the implementation (due to preconditions), but I can do it here in the paper. However, since we quantify over every unconstraint a, I think this is not necessary, eqLabeled or checkLabeled cannot messup with the arguemnts.}

\subsection{Implementation and reproductability}
The complete implementation of these meta programs is about 800 LoC (without blanks, with comments).
Most of the work have been factored and abstracted such that the meta-programs are usable outside of the direct scope of this work.

During our experiments, the API of \gls{metastar} changed a bit, sometimes breaking some of our meta programs.
For a matter of reproducability, we therefore leverage the Nix package manager (\url{https://nixos.org}), that builds specific versions of \gls{fstar} such that our examples work without trouble.

\subsection{Limitations}

\paragraph{Genericity}

The main limitation of our approach is by design: one is not able to spell out a theorem over all programs, but simply the program at hand.

\paragraph{Reification}

Another limitation regards reification, in that programs that can be handled and proven non-interferent are required to lives in an effect that is \textit{reifiable} to a total computation.
For instance, let's consider an effect with a primitive that produces random numbers.
A reifiable model of such an effect would be to admit an infinite stream of numbers as an input of the computation.
Proving properties about a program that uses randomness could then be done by quantifying it universally over this stream.

However, in \gls{fstar}, an effect primitive can also be \textit{assumed} by giving a specification, i.e. a static semantic by means of a dependent-type, but no implementation, that is, no  dynamic semantics.
In such a case, one is able to conduct proofs, but unable to normalize programs (as some primitives have no implementation).
That latter feature is necessary to conduct properly our proofs on generated theorems.

\paragraph{Maturity} 

Finally, C code extraction with \gls{krml} seems not to play nicely with reifiable effect, resulting in copy-paste like quirks in our implementation.
Also, \gls{metastar} is young: the reflected AST of terms in \gls{fstar} is not complete with regards to actual \gls{fstar} terms.
Nonetheless, we have great hope these issues will be relaxed in the future.

\lf{Shouldn't the following two paragraph stay in conclusion? The meta star proof thing, morally, should work on any reifiable effect, layered effect or not, LowStar effect or not.}
\jpc{Way too technical for the conclusion}

\paragraph{Effects} 

Our current implementation of \gls{liostar} only handles pure functions and we do not yet use the \gls{lowstar}'s effects to allow for a complete memory model. There are several  reasons to this design choice: 1/ using \gls{fstar}'s base effects would imply modifying the \gls{lowstar} API to include labels, 2/ the \gls{lowstar} memory API is going to be re-engineered, and 3/ the layered effect is a new way of declaring effect currently being tested in \gls{fstar}.

This last improvement of \gls{fstar} will enable us to define \gls{ifc} effects independently of input/output models and allow to express IFC in a much simpler and elegant way by the composition of effects. This will make our \gls{ifc} library a lot more portable and allow to significantly reduce its \gls{tcb}. 



